Provenance in Temporal Interaction Networks

In temporal interaction networks, vertices correspond to entities, which exchange data quantities (e.g., money, bytes, messages) over time. Tracking the origin of data that have reached a given vertex at any time can help data analysts to understand the reasons behind the accumulated quantity at the vertex or behind the interactions between entities. In this paper, we study data provenance in a temporal interaction network. We investigate alternative propagation models that may apply to different application scenarios. For each such model, we propose annotation mechanisms that track the origin of propagated data in the network and the routes of data quantities. Besides analyzing the space and time complexity of these mechanisms, we propose techniques that reduce their cost in practice, by either (i) limiting provenance tracking to a subset of vertices or groups of vertices, or (ii) tracking provenance only for quantities that were generated in the near past or limiting the provenance data in each vertex by a budget constraint. Our experimental evaluation on five real datasets shows that quantity propagation models based on generation time or receipt order scale well on large graphs; on the other hand, a model that propagates quantities proportionally has high space and time requirements and can benefit from the aforementioned cost reduction techniques.

==> problem.tex <==
\section{Problem}\label{sec:prob}
The input to our problem is a network, which captures the history of
interactions between vertices. For all vertices of the interaction
network (or a given subset of vertices), our goal is to compute the
origin of the quantity that is accumulated to them by the end of the
timeline.

The quantity at each vertex is computed based on the assumption that
each interaction $(q,t)$ from a vertex $v$ to a vertex $u$ transfers
from the accumulated quantity at the source vertex $v$ by time $t$,
either $q$ (if $v$ has at least $q$ units in its buffer) or the entire
accumulated quantity if it is less than $q$. In the latter case, $v$
{\em generates} the difference $q'$, and $q'$ is marked to have $v$ as
its origin as it flows in the network.
Hence, we assume that throughout the history of interactions, each
vertex $v$ has a {\em buffer} $B_v$. At the end of the timeline, $B_v$
represents the total quantity accumulated at $v$ (which was not
relayed).
By accessing all interactions in time order, we can compute the
buffered quantities of all vertices. Our provenance problem is to find
the origin(s) of $B_v$ for each vertex $v$.

If, for an interaction $(q,t)$, the source vertex $v$ has a buffer
$B_v>q$, then it is necessary to select which part of $B_v$ will be
relayed to the destination vertex $u$.
Hence, for the case where $B_v>q$, we study different relay models,
which are based on realistic assumptions:
\begin{itemize}
\item{\em least recently born prioritization:} this model gives
  priority to the quantities that have an oldest birth timestamps. As
  an example, consider the transaction $(6,4)$ shown in Figure
  \ref{fig:oldestfirst} from $v$ to $u$. Assume that, by time $t=6$,
  $B_v=5$, i.e., $q=4 < B_v$. Assume that $B_v$ is analyzed to
  $\{[(x,2),1], [(y,3),2]\}$, meaning that from the total $B_v$, $2$
  units originate from vertex $x$, born at time $1$ and $3$ units
  originate from vertex $y$, born at time $2$. Based on this model,
  $v$ will relay to $u$ the $q=4$ quantity units which are the least
  recently born, i.e., quantities $\{[(x,2),1], [(y,2),2]\}$; hence
  $B_v$ will be updated to $B_v=\{[(y,1),2]\}$.
\item{\em most recently born prioritization:} this is the same as the
  previous model, with the only difference being that priority is
  given to the most recently born quantities.
\item{\em proportional selection:} the transfered quantity is selected
  proportionally, based on the origin. Consider again our previous
  example with transaction $(6,4)$ from vertex $v$ with $B_v=5$
  originate from $x$ and $3$ units originate from $B_v$ to $B_u$.
 \end{itemize}



\textbf{Least Recently Born Prioritization:} The logic behind this
model is the following: when the flow $f$ is transferred from one node
to another, the model gives priopity to the flow that has the oldest
birth timestamp. To understand better the model, consider the example
in Figure \ref{fig:least}. For the interaction $(v,u,8,3)$ 
that happens by time $3$,
the buffer of $v$ is $B_v =\{[(x,4),1], [(y,6),2]\}$, meaning that $v$
has accumulated a quantity of $4$
born at time $1$ at vertex $x$ and a quantity of $6$ born at time $2$
at vertex $y$.
Based on this model, $v$ will relay to $u$ quantities  $\{[(x,4),1],
[(y,4),2]\}$ and $B_v$ will be updated to $B_v =\{[(y,2),2]\}$.
This is because $[(x,4),1]$ is born before $[(y,6),2]$, hence,
$[(x,4),1]$ is relayed first,
and then the remaining quantity $8-4=4$ is taken from $[(y,6),2]$ and subtracted from $B_v$.


\begin{figure}[tbh]
 \centering
 \small
  \includegraphics[width=0.80\columnwidth]{least.pdf}
  \caption{Example of least recently born prioritization model}
  \label{fig:least}
\end{figure}


\textbf{Most Recently Born Prioritization:} This model follows the
same logic as the above model with the only difference being that
priority is given to the most recently born quantities. Consider again
the previous example +++

\textbf{Proportional Selection:} The transfered quantity is selected proportionally, based on the origin.
Consider the interaction $(v,u,5,3)$
and assume that by time $3$, the buffer of $v$ is $B_v =\{[(x,4),1],
[(y,6),2]\}$ in Figure \ref{fig:prop}.
This model will select to relay a quantity of $5$ proportionally from  $[(x,4),1]$ and $[(y,6),2]$, i.e., $2$ will be selected from $[(x,4),1]$ and $3$ will be selected from $[(y,6),2]$. Hence, quantities $\{[(x,2),1], [(y,3),2]\}$ will be added to $B_u$ and $B_v$ will be updated to $\{[(x,2),1], [(y,3),2]\}$.

\textbf{Time-Decayed Proportional Selection:}  Same as the previous
model,
but in the proportional selection larger weight is given to the most recently born quantities.

%\begin{figure}[tbh]
%  \centering
%  \small
%  \includegraphics[width=0.80\columnwidth]{prop.pdf}
%  \caption{Example of proportional selection model}
%  \label{fig:prop}
%\end{figure}





